Relational Semantics for Flat Heyting-Lewis Logic

We introduce relational semantics for "flat Heyting-Lewis logic" HLC-flat. This logic arises as the extension of intuitionistic logic with a Lewis-style strict implication modality that, contrary to its "sharp" counterpart HLC-sharp, does not turn meets into joins in its first argument. We prove completeness and the finite model property for HLC-flat and for several extensions with additional axioms.

==> eptcsdata.tex <==
\providecommand{\firstpage}{445}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.25}{10.4204/EPTCS.447.25}}
\pdfoutput=1

